End-to-End Polyphonic Sound Event Detection Using Convolutional Recurrent Neural Networks with Learned Time-Frequency Representation Input

Sound event detection systems typically consist of two stages: extracting hand-crafted features from the raw audio waveform, and learning a mapping between these features and the target sound events using a classifier. Recently, the focus of sound event detection research has been mostly shifted to the latter stage using standard features such as mel spectrogram as the input for classifiers such as deep neural networks. In this work, we utilize end-to-end approach and propose to combine these two stages in a single deep neural network classifier. The feature extraction over the raw waveform is conducted by a feedforward layer block, whose parameters are initialized to extract the time-frequency representations. The feature extraction parameters are updated during training, resulting with a representation that is optimized for the specific task. This feature extraction block is followed by (and jointly trained with) a convolutional recurrent network, which has recently given state-of-the-art results in many sound recognition tasks. The proposed system does not outperform a convolutional recurrent network with fixed hand-crafted features. The final magnitude spectrum characteristics of the feature extraction block parameters indicate that the most relevant information for the given task is contained in 0 - 3 kHz frequency range, and this is also supported by the empirical results on the SED performance.

==> table_results.tex <==
\begin{tabular}{ @{} l *{1}{c c }} 
\toprule 
% & \multicolumn{4}{c|}{TUT-SED Synthetic 2016} &\multicolumn{4}{c|}{TUT-SED 2009} & \multicolumn{4}{c}{TUT-SED 2016}\\

Method & $F1_{\textnormal{frm}}$ & $ER_{\textnormal{frm}}$ \\
\midrule

% DFT 8 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% DFT 8 kHz learned 					& 60.8$\pm$0.8 &0.48$\pm$0.01 \\
% Mel 8 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Mel 8 kHz learned 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Log mel 8 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Log mel 8 kHz learned 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% DFT 8 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% DFT 8 kHz learned 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Mel 16 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Mel 16 kHz learned 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Log mel 16 kHz fixed 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Log mel 16 kHz learned 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
% Log mel 44.1 kHz fixed~\cite{emre_TASLP2016} 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\
DFT 8 kHz fixed 					& 60.8$\pm$0.8 &0.55$\pm$0.01 \\
Mel 8 kHz fixed 					& 60.8$\pm$0.9 &0.55$\pm$0.01 \\
Log mel 8 kHz fixed 					& 63.1$\pm$0.6 &0.52$\pm$0.01 \\
DFT 16 kHz fixed 					& 61.9$\pm$0.9 &0.54$\pm$0.01 \\
Mel 16 kHz fixed 					& 62.3$\pm$0.7 &0.54$\pm$0.01 \\
Log mel 16 kHz fixed 					& 65.8$\pm$1.4 &0.50$\pm$0.01 \\
\midrule
DFT 8 kHz learned 					& 60.8$\pm$0.8 &0.55$\pm$0.01 \\
Mel 8 kHz learned 					& 61.0$\pm$0.8 &0.56$\pm$0.01 \\
Log mel 8 kHz learned 					& 58.6$\pm$1.6 &0.56$\pm$0.01 \\
DFT 16 kHz learned 					& 60.1$\pm$1.7 &0.58$\pm$0.03 \\
Mel 16 kHz learned 					& 60.6$\pm$0.9 &0.57$\pm$0.02 \\
Log mel 16 kHz learned 					& 59.9$\pm$1.3 &0.56$\pm$0.01 \\
DFT 24 kHz learned 					& 58.1$\pm$1.6 &0.59$\pm$0.03 \\
\midrule


Log mel 44.1 kHz fixed~\cite{emre_TASLP2016} 					& 66.4$\pm$0.6 &0.48$\pm$0.01 \\

\bottomrule
\end{tabular}
